Sparsity Winning Twice: Better Robust Generalization from More Efficient Training

Recent studies demonstrate that deep networks, even robustified by the state-of-the-art adversarial training (AT), still suffer from large robust generalization gaps, in addition to the much more expensive training costs than standard training. In this paper, we investigate this intriguing problem from a new perspective, i.e., injecting appropriate forms of sparsity during adversarial training. We introduce two alternatives for sparse adversarial training: (i) static sparsity, by leveraging recent results from the lottery ticket hypothesis to identify critical sparse subnetworks arising from the early training; (ii) dynamic sparsity, by allowing the sparse subnetwork to adaptively adjust its connectivity pattern (while sticking to the same sparsity ratio) throughout training. We find both static and dynamic sparse methods to yield win-win: substantially shrinking the robust generalization gap and alleviating the robust overfitting, meanwhile significantly saving training and inference FLOPs. Extensive experiments validate our proposals with multiple network architectures on diverse datasets, including CIFAR-10/100 and Tiny-ImageNet. For example, our methods reduce robust generalization gap and overfitting by 34.44% and 4.02%, with comparable robust/standard accuracy boosts and 87.83%/87.82% training/inference FLOPs savings on CIFAR-100 with ResNet-18. Besides, our approaches can be organically combined with existing regularizers, establishing new state-of-the-art results in AT. Codes are available in https://github.com/VITA-Group/Sparsity-Win-Robust-Generalization.

==> Table1.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[htbp]
  \centering
  \caption{Results of robust train of different sparsity. We compared several different ways to achieve the specified sparsity. The checkpoint is picked which has the best valid robust accuracy. }
    \begin{tabular}{c|c|rrr|rrr|rrr}
    \toprule
    \multirow{2}[2]{*}{Density} & \multirow{2}[2]{*}{Setting} & \multicolumn{3}{c|}{Roubst Accuarcy(RA)} & \multicolumn{3}{c|}{Standard Accuarcy(RA)} & \multicolumn{3}{c}{Generalization Gap} \\
          &       & \multicolumn{1}{c}{Best} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c|}{Diff.} & \multicolumn{1}{c}{Best} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c|}{Diff.} & \multicolumn{1}{c}{Best} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{Diff.} \\
    \midrule
    1     & dense & 51.95 & 43.59 & 8.36  & 80.9  & 83.69 & -2.79 & 7.43  & 42.17 & -34.74 \\
    \midrule
    \multirow{5}[2]{*}{0.8} & small dense & 50.43 & 42.69 & 7.74  & 80.73 & 82.76 & -2.03 & 7.14  & 40.16 & -33.02 \\
          & omp   & 52.16 & 43.72 & \multicolumn{1}{r}{8.44} & 80.6  & 83.53 & \multicolumn{1}{r}{-2.93} & 6.92  & 40.68 & -33.76 \\
          & rp    & 51.32 & 43.42 & \multicolumn{1}{r}{7.9} & 81.03 & 82.99 & \multicolumn{1}{r}{-1.96} & 7.96  & 40.48 & -32.52 \\
          & dst random & 51.47 & 41.52 & 9.95  & 82.23 & 83.07 & -0.84 & 8.59  & 43.52 & -34.93 \\
          &  dst gradient & 51.44 & 43.94 & 7.5   & 80.47 & 83.55 & -3.08 & 3.92  & 40.94 & -37.02 \\
    \midrule
    \multirow{5}[2]{*}{0.6} & small dense & 50.66 & 43.03 & 7.63  & 80.31 & 82.97 & -2.66 & 7.23  & 36.15 & -28.92 \\
          & omp   & 51.52 & 43.93 & 7.59  & 81.14 & 83.27 & -2.13 & 7.81  & 38.42 & -30.61 \\
          & rp    & 51.37 & 43.5  & 7.87  & 80.5  & 82.48 & -1.98 & 7.15  & 38.1  & -30.95 \\
          & dst random & 51.38 & 43.54 & 7.84  & 81.13 & 82.87 & -1.74 & 7.58  & 40.46 & -32.88 \\
          &  dst gradient & 52.08 & 43.73 & 8.35  & 81.19 & 83.88 & -2.69 & 7.98  & 40.01 & -32.03 \\
    \midrule
    \multirow{5}[2]{*}{0.2} & small dense & 49.04 & 44.18 & 4.86  & 76.64 & 80.77 & -4.13 & 3.68  & 20.77 & -17.09 \\
          & omp   & 50.16 & 45.02 & 5.14  & 79.8  & 82.39 & -2.59 & 5.72  & 26.28 & -20.56 \\
          & rp    & 49.32 & 43.97 & 5.35  & 77.75 & 81.27 & -3.52 & 4.22  & 23.26 & -19.04 \\
          & dst random & 50.82 & 45.66 & 5.16  & 82.37 & 83.6  & -1.23 & 9.2   & 28.9  & -19.7 \\
          &  dst gradient & 51.62 & 46.37 & 5.25  & 80.55 & 83.17 & -2.62 & 6.48  & 27.19 & -20.71 \\
    \midrule
    \multirow{5}[1]{*}{0.1} & small dense & 46.81 & 45.48 & 1.33  & 77.13 & 78.54 & -1.41 & 8.48  & 12.34 & -3.86 \\
          & omp   & 49.31 & 46.11 & 3.2   & 77.99 & 81    & -3.01 & 3.79  & 17.55 & -13.76 \\
          & rp    & 47.09 & 44.97 & 2.12  & 75.25 & 78.77 & -3.52 & 3.67  & 13.44 & -9.77 \\
          & dst random & 50.86 & 47.1  & 3.76  & 80.57 & 82.67 & -2.1  & 5.87  & 20.23 & -14.36 \\
          &  dst gradient & 50.97 & 48.1  & 2.87  & 79.62 & 82.93 & -3.31 & 5.01  & 18.44 & -13.43 \\
    \midrule
    \multirow{5}[1]{*}{0.05} & small dense & 45.99 & 44.55 & 1.44  & 74.26 & 75.64 & -1.38 & 5.37  & 7.67  & -2.3 \\
          & omp   & 47.08 & 46.23 & 0.85  & 78.77 & 79.36 & -0.59 & 7.94  & 10.39 & -2.45 \\
          & rp    & 45.64 & 44.18 & 1.46  & 75.2  & 75.2  & 0     & 4.86  & 7.08  & -2.22 \\
          & dst random & 49.61 & 47.71 & 1.9   & 80.8  & 81.71 & -0.91 & 9.81  & 13.39 & -3.58 \\
          &  dst gradient & 50.17 & 49.18 & 0.99  & 78.12 & 81.43 & -3.31 & 3.71  & 11.23 & -7.52 \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> Tables/Table1.tex <==
% Table generated by Excel2LaTeX from sheet 'Table1'
\begin{table}[htbp]
  \centering
  \caption{Results of robust train of different sparsity. We compared several different ways to achieve the specified sparsity. The checkpoint is picked which has the best valid robust accuracy.}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|ccc|ccc|ccc|c}
    \toprule
    \multirow{2}[2]{*}{Density} & \multirow{2}[2]{*}{Setting} & \multicolumn{3}{c|}{Roubst Accuarcy(RA)} & \multicolumn{3}{c|}{Standard Accuarcy(RA)} & \multicolumn{3}{c|}{Generalization Gap} & \multirow{2}[2]{*}{final density(\%)} \\
          &       & Best  & Final & Diff. & Best  & Final & Diff. & Best  & Final & Diff. &  \\
    \midrule
    1     & dense & \multicolumn{1}{r}{51.95} & \multicolumn{1}{r}{43.59} & \multicolumn{1}{r|}{8.36} & \multicolumn{1}{r}{80.9} & \multicolumn{1}{r}{83.69} & \multicolumn{1}{r|}{-2.79} & \multicolumn{1}{r}{7.43} & \multicolumn{1}{r}{42.17} & \multicolumn{1}{r|}{-34.74} & 100 \\
    \midrule
    \multirow{10}[2]{*}{0.8} & small dense & 50.43 & 42.69 & 7.74  & 80.73 & 82.76 & -2.03 & 7.14  & 40.16 & -33.02 & 80 \\
          & omp   & 52.16 & 43.72 & 8.44  & 80.6  & 83.53 & -2.93 & 6.92  & 40.68 & -33.76 & 80 \\
          & rp    & 51.32 & 43.42 & 7.9   & 81.03 & 82.99 & -1.96 & 7.96  & 40.48 & -32.52 & 80 \\
          & snip  & 51.98 & 43.71 & 8.27  & 81.57 & 83.56 & -1.99 & 7.84  & 40.71 & -32.87 & 80 \\
          & grasp & 51.48 & 42.98 & 8.5   & 80.61 & 83.23 & -2.62 & 6.62  & 40.48 & -33.86 & 80 \\
          & synflow & 51.68 & 44.55 & 7.13  & 81.01 & 83.08 & -2.07 & 7.75  & 38.79 & -31.04 & 80 \\
          & igq   & 52.04 & 43.73 & 8.31  & 81.44 & 83.17 & -1.73 & 7.79  & 40.68 & -32.89 & 80 \\
          & dst random & 51.47 & 41.52 & 9.95  & 82.23 & 83.07 & -0.84 & 8.59  & 43.52 & -34.93 & 80 \\
          &  dst gradient & 51.44 & 43.94 & 7.5   & 80.47 & 83.55 & -3.08 & 3.92  & 40.94 & -37.02 & 80 \\
          & flying & 50.8  & 42.76 & 8.04  & 82.5  & 83.25 & -0.75 & 9.5   & 39.1  & -29.6 & 39.34 \\
    \midrule
    \multirow{10}[2]{*}{0.6} & small dense & 50.66 & 43.03 & 7.63  & 80.31 & 82.97 & -2.66 & 7.23  & 36.15 & -28.92 & 60 \\
          & omp   & 51.52 & 43.93 & 7.59  & 81.14 & 83.27 & -2.13 & 7.81  & 38.42 & -30.61 & 60 \\
          & rp    & 51.37 & 43.5  & 7.87  & 80.5  & 82.48 & -1.98 & 7.15  & 38.1  & -30.95 & 60 \\
          & snip  & 52.06 & 43.8  & 8.26  & 80.9  & 83.51 & -2.61 & 6.91  & 38.22 & -31.31 & 60 \\
          & grasp & 51.15 & 43.28 & 7.87  & 80.36 & 82.43 & -2.07 & 6.96  & 37.78 & -30.82 & 60 \\
          & synflow & 51.67 & 44.07 & 7.6   & 81.04 & 83.7  & -2.66 & 7.77  & 37.58 & -29.81 & 60 \\
          & igq   & 51.48 & 43.82 & 7.66  & 81.41 & 83.36 & -1.95 & 7.83  & 38.41 & -30.58 & 60 \\
          & dst random & 51.38 & 43.54 & 7.84  & 81.13 & 82.87 & -1.74 & 7.58  & 40.46 & -32.88 & 60 \\
          &  dst gradient & 52.08 & 43.73 & 8.35  & 81.19 & 83.88 & -2.69 & 7.98  & 40.01 & -32.03 & 60 \\
          & flying & 50.56 & 44.23 & 6.33  & 82.18 & 83.12 & -0.94 & 9.71  & 35.91 & -26.2 & 28.67 \\
    \midrule
    \multirow{10}[2]{*}{0.2} & small dense & 49.04 & 44.18 & 4.86  & 76.64 & 80.77 & -4.13 & 3.68  & 20.77 & -17.09 & 20 \\
          & omp   & 50.16 & 45.02 & 5.14  & 79.8  & 82.39 & -2.59 & 5.72  & 26.28 & -20.56 & 20 \\
          & rp    & 49.32 & 43.97 & 5.35  & 77.75 & 81.27 & -3.52 & 4.22  & 23.26 & -19.04 & 20 \\
          & snip  & 50.46 & 46.44 & 4.02  & 80.13 & 83.2  & -3.07 & 5.55  & 23.37 & -17.82 & 20 \\
          & grasp & 50.16 & 45.31 & 4.85  & 78.38 & 82.42 & -4.04 & 4.43  & 24.27 & -19.84 & 20 \\
          & synflow & 51.17 & 46.91 & 4.26  & 79.08 & 83.19 & -4.11 & 3.97  & 22.52 & -18.55 & 20 \\
          & igq   & 51.12 & 46.74 & 4.38  & 79.73 & 83.26 & -3.53 & 4.71  & 23.43 & -18.72 & 20 \\
          & dst random & 50.82 & 45.66 & 5.16  & 82.37 & 83.6  & -1.23 & 9.2   & 28.9  & -19.7 & 20 \\
          &  dst gradient & 51.62 & 46.37 & 5.25  & 80.55 & 83.17 & -2.62 & 6.48  & 27.19 & -20.71 & 20 \\
          & flying & 51.7  & 47.51 & 4.19  & 80.74 & 83.16 & -2.42 & 6.53  & 22.11 & -15.58 & 10.03 \\
    \midrule
    \multirow{10}[2]{*}{0.1} & small dense & 46.81 & 45.48 & 1.33  & 77.13 & 78.54 & -1.41 & 8.48  & 12.34 & -3.86 & 10 \\
          & omp   & 49.31 & 46.11 & 3.2   & 77.99 & 81    & -3.01 & 3.79  & 17.55 & -13.76 & 10 \\
          & rp    & 47.09 & 44.97 & 2.12  & 75.25 & 78.77 & -3.52 & 3.67  & 13.44 & -9.77 & 10 \\
          & snip  & 49.49 & 47.85 & 1.64  & 77.74 & 81.92 & -4.18 & 3.29  & 14.39 & -11.1 & 10 \\
          & grasp & 48.56 & 46.8  & 1.76  & 79.02 & 81.39 & -2.37 & 5.28  & 15.45 & -10.17 & 10 \\
          & synflow & 50.08 & 48.02 & 2.06  & 81.15 & 81.56 & -0.41 & 10.22 & 13.39 & -3.17 & 10 \\
          & igq   & 49.74 & 48.05 & 1.69  & 81.06 & 81.84 & -0.78 & 9.86  & 14.47 & -4.61 & 10 \\
          & dst random & 50.86 & 47.1  & 3.76  & 80.57 & 82.67 & -2.1  & 5.87  & 20.23 & -14.36 & 10 \\
          &  dst gradient & 50.97 & 48.1  & 2.87  & 79.62 & 82.93 & -3.31 & 5.01  & 18.44 & -13.43 & 10 \\
          & flying & 50.88 & 49.27 & 1.61  & 79.95 & 82.65 & -2.7  & 5.78  & 13.82 & -8.04 & 4.73 \\
    \midrule
    \multirow{10}[2]{*}{0.05} & small dense & 45.99 & 44.55 & 1.44  & 74.26 & 75.64 & -1.38 & 5.37  & 7.67  & -2.3  & 5 \\
          & omp   & 47.08 & 46.23 & 0.85  & 78.77 & 79.36 & -0.59 & 7.94  & 10.39 & -2.45 & 5 \\
          & rp    & 45.64 & 44.18 & 1.46  & 75.2  & 75.2  & 0     & 4.86  & 7.08  & -2.22 & 5 \\
          & snip  & 48.18 & 46.72 & 1.46  & 78.55 & 79.21 & -0.66 & 6.48  & 8.43  & -1.95 & 5 \\
          & grasp & 48.58 & 47.15 & 1.43  & 78.95 & 79.44 & -0.49 & 6.86  & 8.89  & -2.03 & 5 \\
          & synflow & 48.93 & 48.22 & 0.71  & 78.7  & 78.9  & -0.2  & 5.83  & 7.18  & -1.35 & 5 \\
          & igq   & 48.82 & 47.56 & 1.26  & 79.44 & 79.76 & -0.32 & 6.46  & 8.51  & -2.05 & 5 \\
          & dst random & 49.61 & 47.71 & 1.9   & 80.8  & 81.71 & -0.91 & 9.81  & 13.39 & -3.58 & 5 \\
          &  dst gradient & 50.17 & 49.18 & 0.99  & 78.12 & 81.43 & -3.31 & 3.71  & 11.23 & -7.52 & 5 \\
          & flying & 49.37 & 48.84 & 0.53  & 80.33 & 80.28 & 0.05  & 8     & 9.11  & -1.11 & 2.68 \\
    \bottomrule
    \end{tabular}}
  \label{tab:addlabel}%
\end{table}%


==> Tables/batch.tex <==
% Table generated by Excel2LaTeX from sheet 'batch'
\begin{table}[htbp]
  \centering
  \caption{The ablation study of batch size.}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|ccc|ccc|ccc|c|c}
    \toprule
    \multirow{2}[2]{*}{Batch Size} & \multicolumn{3}{c|}{Roubst Accuarcy(RA)} & \multicolumn{3}{c|}{Standard Accuarcy(RA)} & \multicolumn{3}{c|}{Generalization Gap} & \multirow{2}[2]{*}{Sparsity} & \multirow{2}[2]{*}{Total Fired Weights} \\
          & Best  & Final & Diff. & Best  & Final & Diff. & Best  & Final & Diff. &       &  \\
    \midrule
    32    & 48.46 & 47.77 & 0.69  & 78.03 & 78.65 & -0.62 & 4.29  & 4.86  & -0.57 & 1.66  & 0.55 \\
    64    & 49.08 & 47.44 & 1.64  & 80.51 & 80.58 & -0.07 & 9.51  & 11.14 & -1.63 & 2.73  & 0.59 \\
    128   & 50.88 & 49.27 & 1.61  & 79.95 & 82.65 & -2.7  & 5.78  & 13.82 & -8.04 & 4.73  & 0.55 \\
    256   & 50.06 & 47.79 & 2.27  & 81    & 82.21 & -1.21 & 9.91  & 18.13 & -8.22 & 6.93  & 0.44 \\
    512   & 49.68 & 46.49 & 3.19  & 80.41 & 81.78 & -1.37 & 9.58  & 19.91 & -10.33 & 8.58  & 0.33 \\
    \bottomrule
    \end{tabular}}
  \label{tab:addlabel}%
\end{table}%


==> Tables/init.tex <==
% Table generated by Excel2LaTeX from sheet 'init'
\begin{table}[htbp]
  \centering
  \caption{The ablation study of sparsity initialization.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|ccc|ccc|ccc|c|c}
    \toprule
    \multirow{2}[2]{*}{Initialization} & \multicolumn{3}{c|}{Roubst Accuarcy(RA)} & \multicolumn{3}{c|}{Standard Accuarcy(RA)} & \multicolumn{3}{c|}{Generalization Gap} & \multirow{2}[2]{*}{Sparsity} & \multirow{2}[2]{*}{Total Fired Weights} \\
          & Best  & Final & Diff. & Best  & Final & Diff. & Best  & Final & Diff. &       &  \\
    \midrule
    Uniform & 49.09 & 46.96 & 2.13  & 78.32 & 80.32 & -2    & 5.37  & 14.03 & -8.66 & 4.35  & 0.66 \\
    Snip  & 51.3  & 49.17 & 2.13  & 79.86 & 82.28 & -2.42 & 4.66  & 13.72 & -9.06 & 4.46  & 0.41 \\
    Igq   & 50.88 & 49.27 & 1.61  & 79.95 & 82.65 & -2.7  & 5.78  & 13.82 & -8.04 & 4.73  & 0.55 \\
    fixed ERK & 50.57 & 47.7  & 2.87  & 79.53 & 82.21 & -2.68 & 5.52  & 17.15 & -11.63 & 7.3   & 0.6 \\
    SynFlow & 50.56 & 48.75 & 1.81  & 78.51 & 82.17 & -3.66 & 3.98  & 12.85 & -8.87 & 4.76  & 0.26 \\
    \bottomrule
    \end{tabular}}
  \label{tab:addlabel}%
\end{table}%


==> Tables/res18_cifar100.tex <==
% Table generated by Excel2LaTeX from sheet 'res18_cifar100'
\begin{table}[htbp]
  \centering
  \caption{Resnet18 Cifar100}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|ccc|ccc|ccc|c}
    \toprule
    \multirow{2}[2]{*}{Density} & \multirow{2}[2]{*}{Setting} & \multicolumn{3}{c|}{Roubst Accuarcy(RA)} & \multicolumn{3}{c|}{Standard Accuarcy(RA)} & \multicolumn{3}{c|}{Generalization Gap} & \multirow{2}[2]{*}{final density(\%)} \\
          &       & Best  & Final & Diff. & Best  & Final & Diff. & Best  & Final & Diff. &  \\
    \midrule
    1     & dense & 26.93 & 19.62 & 7.31  & 52.03 & 53.91 & -1.88 & 5.06  & 56.41 & -51.35 & 100 \\
    \midrule
    \multirow{8}[1]{*}{0.2} & omp   & 25.12 & 20.18 & 4.94  & 50.08 & 52.81 & -2.73 & 6.35  & 30.23 & -23.88 & 20 \\
          & rp    & 25.92 & 20.83 & 5.09  & 48.16 & 51.31 & -3.15 & 3.01  & 30.31 & -27.3 & 20 \\
          & snip  & 26.61 & 23.55 & 3.06  & 49.47 & 54.79 & -5.32 & 2.39  & 22.78 & -20.39 & 20 \\
          & grasp & 25.37 & 20.79 & 4.58  & 50.27 & 53.29 & -3.02 & 6     & 29.83 & -23.83 & 20 \\
          & synflow & 26.31 & 23.52 & 2.79  & 48.33 & 54.49 & -6.16 & 1.99  & 19.5  & -17.51 & 20 \\
          & igq   & 26.87 & 23.07 & 3.8   & 49.8  & 54.39 & -4.59 & 2.59  & 25.75 & -23.16 & 20 \\
          &  dst gradient & 26.64 & 22    & 4.64  & 53.57 & 55.41 & -1.84 & 8.42  & 29.68 & -21.26 & 20 \\
          & flying & 26.66 & 23.37 & 3.29  & 52.29 & 55.23 & -2.94 & 7.12  & 21.82 & -14.7 & 8.51 \\
    \midrule
    \multirow{8}[2]{*}{0.1} & omp   & 24.45 & 21.38 & 3.07  & 48.02 & 51.26 & -3.24 & 4.24  & 18.37 & -14.13 & 10 \\
          & rp    & 24.06 & 21.45 & 2.61  & 47.06 & 49.73 & -2.67 & 2.66  & 17.42 & -14.76 & 10 \\
          & snip  & 26.1  & 24.46 & 1.64  & 52.35 & 52.88 & -0.53 & 7.42  & 10.73 & -3.31 & 10 \\
          & grasp & 24.83 & 22.74 & 2.09  & 51.09 & 52.55 & -1.46 & 10.41 & 15.36 & -4.95 & 10 \\
          & synflow & 25.45 & 24.62 & 0.83  & 51.03 & 51.96 & -0.93 & 6.84  & 9.32  & -2.48 & 10 \\
          & igq   & 26.22 & 24.87 & 1.35  & 52.37 & 53.16 & -0.79 & 9.04  & 12.55 & -3.51 & 10 \\
          &  dst gradient & 26.14 & 23.57 & 2.57  & 50.53 & 54.78 & -4.25 & 3.78  & 17.69 & -13.91 & 10 \\
          & flying & 26.26 & 24.16 & 2.1   & 51.16 & 53.97 & -2.81 & 4.31  & 12.56 & -8.25 & 4.08 \\
    \bottomrule
    \end{tabular}}
  \label{tab:addlabel}%
\end{table}%


==> Tables/robust_bird.tex <==
\begin{table}[htbp]
  \centering
  \caption{Robust Bird: Resnet18 CIFAR 10 }
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|ccc|ccc|ccc|c}
    \toprule
    \multirow{2}[2]{*}{Density} & \multirow{2}[2]{*}{Setting} & \multicolumn{3}{c|}{Roubst Accuarcy(RA)} & \multicolumn{3}{c|}{Standard Accuarcy(RA)} & \multicolumn{3}{c|}{Generalization Gap} & \multirow{2}[2]{*}{final density(\%)} \\
          &       & Best  & Final & Diff. & Best  & Final & Diff. & Best  & Final & Diff. &  \\

    \midrule
    \multirow{3}[1]{*}{1} 
& sgd+pgd & 51.47	& 42.68	& 8.79	& 83.59	& 82.72	& 0.87	& 28.34	& 37.13	& -8.79 & \\
& fast+pgd & 51.99	& 43.38	& 8.61	& 83.85	& 82.77	& 1.08	& 38.39	& 47.00	& -8.61 &  \\
& pgd+pgd & 52.16	& 42.81	& 9.35	& 83.85	& 82.93	& 0.92	& 36.08	& 45.43	& -9.35 &  \\

    \multirow{3}[1]{*}{1} 
& sgd(rb)+pgd & 51.98 & 42.18 & 9.8   & 83.47 & 82.85 & 0.62 & 36.42 & 46.12 & -9.71  & \\
& fast(rb)+pgd & 51.91 & 41.63 & 10.28 & 83.41 & 82.83 & 0.58 & 37.87 & 48.15 & -10.28 & \\
& pgd(rb)+pgd & 51.92 & 42.19 & 9.73  & 83.69 & 82.81 & 0.88 & 38.06 & 47.62 & -9.56  & \\
    \midrule


    \multirow{3}[1]{*}{0.8} 
&  sgd+pgd  & 51.77	& 43.23	& 8.54	& 83.52	& 82.73	& 0.79	& 28.39	& 36.87	& -8.49 & \\
& fast+pgd & 51.93	& 43.09	& 8.84	& 83.99	& 83.10	& 0.89	& 37.95	& 46.79	& -8.84 & \\
& pgd+ pgd & 51.98	& 43.73	& 8.25	& 83.80	& 82.93	& 0.87	& 36.06	& 44.30	& -8.24 & \\

    \multirow{3}[1]{*}{0.8} 
& sgd(rb)+pgd & 51.56 & 43.38 & 8.18  & 83.85 & 83.27 & 0.58 & 30.71 & 38.89 & -8.18 & \\
& fast(rb)+pgd & 52.02 & 41.96 & 10.06 & 83.42 & 82.8  & 0.62 & 36.28 & 46.27 & -9.99  & \\
& pgd(rb)+pgd & 52.11 & 41.82 & 10.29 & 83.57 & 82.79 & 0.78 & 37.76 & 48.05 & -10.29 & \\
    \midrule

    
    
    

    \multirow{3}[1]{*}{0.6} 
& sgd+pgd & 51.58	& 43.5	& 8.08	& 83.68	& 82.75	& 0.93	& 28.23	& 36.02	& -7.79 & \\
& fast+pgd & 51.90	& 42.90	& 9.00	& 84.26	& 83.11	& 1.15	& 36.53	& 45.43	& -8.90 & \\
& pgd+pgd & 51.64	& 42.92	& 8.72	& 83.56	& 82.82	& 0.74	& 37.17	& 45.89	& -8.72 & \\

    \multirow{3}[1]{*}{0.6} 
& sgd(rb)+pgd & 51.81 & 42.81 & 9.00 & 84.14 & 83.41 & 0.73 & 29.13 & 38.06 & -8.93 &  \\
& fast(rb)+pgd & 51.61 & 42.07 & 9.54  & 83.47 & 82.5  & 0.97 & 34.14 & 43.47 & -9.34  & \\
& pgd(rb)+pgd & 51.79 & 42.13 & 9.66  & 83.69 & 83.18 & 0.51 & 36.36 & 46.02 & -9.66  & \\
    \midrule
    
    
    \multirow{3}[1]{*}{0.2} 
& sgd+pgd & 51.05	& 44.62	& 6.43	& 83.83	& 83.12	& 0.71	& 23.30	& 29.43	& -6.13 & \\
& fast+pgd & 51.65	& 45.19	& 6.46	& 84.66	& 83.71	& 0.95	& 25.67	& 31.94	& -6.26 & \\
& pgd+pgd & 51.04	& 41.81	& 9.23	& 83.42	& 82.02	& 1.40	& 35.84	& 45.07	& -9.22 & \\

    \multirow{3}[1]{*}{0.2} 
& sgd(rb)+pgd & 50.73 & 43.58 & 7.15  & 83.78 & 83.15 & 0.63 & 22.23 & 29.23 & -7.00 &  \\
& fast(rb)+pgd & 50.58 & 43.68 & 6.9   & 82.95 & 82.29 & 0.66 & 21.59 & 28.4  & -6.8  &  \\
& pgd(rb)+pgd & 50.54 & 43.21 & 7.33  & 82.82 & 81.96 & 0.86 & 22.64 & 29.97 & -7.33  & \\
    \midrule
    

    \multirow{3}[1]{*}{0.1}   
& sgd+pgd & 49.69	& 45.69	& 4.00	& 82.80	& 81.78	& 1.01	& 17.25	& 21.00	& -3.74 & \\
& fast+pgd & 51.43	& 46.81	& 4.62	& 85.10	& 83.94	& 1.16	& 17.89	& 22.18	& -4.29 & \\
& pgd+pgd &  50.16	& 42.80	& 7.36	& 83.46	& 82.28	& 1.18	& 25.54	& 32.90	& -7.35 & \\

    \multirow{3}[1]{*}{0.1}   
& sgd(rb)+pgd & 49.81 & 44.9  & 4.91  & 82.3  & 81.14 & 1.16 & 14.68 & 19.4  & -4.72 &  \\
& fast(rb)+pgd & 49.21 & 44.9  & 4.31  & 81.87 & 81.17 & 0.7  & 14.12 & 18.43 & -4.31  & \\
& pgd(rb)+pgd & 49.45 & 44.99 & 4.46  & 82.1  & 80.95 & 1.15 & 14.62 & 19.08 & -4.46  & \\
    \midrule
    


    \multirow{3}[1]{*}{0.05}   
& sgd+pgd & 10	& 10	& 0	& 10 & 	10	& 0	& 0.21	& -0.26	& 0.48 & \\
& fast+pgd & 49.39	& 48.26	& 1.13	& 82.99	& 82.01	& 0.98	& 10.14	& 11.05	& -0.91 & \\
& pgd+pgd & 49.14	& 45.84	& 3.3	& 82.49	& 81.58	& 0.91	& 13.51	& 16.81	& -3.3 & \\

& sgd(rb)+pgd & 48.46 & 46.52 & 1.94  & 80.79 & 79.82 & 0.97 & 9.05  & 10.99 & -1.94 & \\
& fast(rb)+pgd & 48.95 & 46.12 & 2.83  & 79.83 & 79.09 & 0.74 & 7.51  & 10.34 & -2.83 &  \\
& pgd(rb)+pgd & 48.54 & 46.15 & 2.39  & 80.21 & 78.97 & 1.24 & 8.49  & 10.86 & -2.37  & \\
    \midrule

    \bottomrule
    \end{tabular}}
  \label{tab:rb_ticket_c10_dense}%
\end{table}%






% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  CIFAR-100
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%














\begin{table}[htbp]
  \centering
  \caption{Robust Bird: Resnet18 CIFAR 100 }
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|ccc|ccc|ccc|c}
    \toprule
    \multirow{2}[2]{*}{Density} & \multirow{2}[2]{*}{Setting} & \multicolumn{3}{c|}{Roubst Accuarcy(RA)} & \multicolumn{3}{c|}{Standard Accuarcy(RA)} & \multicolumn{3}{c|}{Generalization Gap} & \multirow{2}[2]{*}{final density(\%)} \\
          &       & Best  & Final & Diff. & Best  & Final & Diff. & Best  & Final & Diff. &  \\

    \midrule
    \multirow{3}[1]{*}{1} 
& sgd+pgd  & 26.7  & 19.17 & 7.53 & 54.04 & 52.4  & 1.64 & 49.84 & 57.13 & -7.29 \\
& fast+pgd & 27.33 & 19.55 & 7.78 & 54.82 & 52.6  & 2.22 & 57.23 & 64.9  & -7.68 \\
& pgd+pgd  & 27.23 & 19.49 & 7.74 & 54.41 & 52.69 & 1.72 & 56.43 & 63.98 & -7.54 \\

    \multirow{3}[1]{*}{1} 
& sgd(rb)+pgd  & 27.09 & 18.9  & 8.19 & 54.61 & 52.85 & 1.76 & 56.86 & 64.96 & -8.1  \\
& fast(rb)+pgd & 27.00 & 19.35 & 7.65 & 53.63 & 52.73 & 0.9  & 56.64 & 64.19 & -7.56 \\
& pgd(rb)+pgd  & 27.03 & 18.92 & 8.11 & 54.23 & 52.67 & 1.56 & 56.64 & 64.75 & -8.1  \\
    \midrule


    \multirow{3}[1]{*}{0.8} 
& sgd+pgd  & 26.82 & 19.06 & 7.76 & 53.76 & 52.6  & 1.16 & 46.76 & 54.37 & -7.6  \\
& fast+pgd & 27.26 & 19.29 & 7.97 & 54.82 & 52.76 & 2.06 & 55.7  & 63.58 & -7.87 \\
& pgd+pgd  & 27.3  & 19.22 & 8.08 & 54.66 & 52.03 & 2.63 & 56.43 & 64.39 & -7.96 \\

    \multirow{3}[1]{*}{0.8} 
& sgd(rb)+pgd  & 27.46 & 19.4  & 8.06 & 55.03 & 52.25 & 2.78 & 54.29 & 62.35 & -8.06 \\
& fast(rb)+pgd & 27.05 & 19.07 & 7.98 & 53.45 & 52.68 & 0.77 & 54.21 & 61.79 & -7.58 \\
& pgd(rb)+pgd  & 27.79 & 19.07 & 8.72 & 54.83 & 52.04 & 2.79 & 55.17 & 63.89 & -8.72 \\
    \midrule

    
    
    

    \multirow{3}[1]{*}{0.6} 
& sgd+pgd  & 27.13 & 19.01 & 8.12 & 54.19 & 52.55 & 1.64 & 42.1  & 50.05 & -7.94 \\
& fast+pgd & 27.3  & 19.57 & 7.73 & 55.09 & 52.48 & 2.61 & 51.56 & 59.29 & -7.72 \\
& pgd+pgd  & 27.23 & 18.69 & 8.54 & 55.11 & 52.03 & 3.08 & 57.61 & 65.91 & -8.3  \\

    \multirow{3}[1]{*}{0.6} 
& sgd(rb)+pgd  & 27.42 & 19.74 & 7.68 & 55.29 & 52.28 & 3.01 & 49.92 & 57.6  & -7.68 \\
& fast(rb)+pgd & 27.13 & 18.57 & 8.56 & 53.38 & 52.5  & 0.88 & 50.27 & 58.83 & -8.56 \\
& pgd(rb)+pgd  & 27.28 & 19.42 & 7.86 & 54.54 & 52.23 & 2.31 & 51.9  & 59.76 & -7.86 \\
    \midrule
    
    
    \multirow{3}[1]{*}{0.2} 
& sgd+pgd  & 26.33 & 20.2  & 6.13 & 54.1  & 52.6  & 1.5  & 25.92 & 31.94 & -6.02 \\
& fast+pgd & 27.50  & 21.15 & 6.35 & 55.93 & 54.42 & 1.51 & 29.02 & 35.37 & -6.35 \\
& pgd+pgd  & 26.21 & 18.18 & 8.03 & 54.73 & 51.65 & 3.08 & 51.74 & 59.5  & -7.76 \\

    \multirow{3}[1]{*}{0.2} 
& sgd(rb)+pgd  & 27.17 & 20.82 & 6.35 & 55.36 & 53.94 & 1.42 & 26.62 & 32.74 & -6.12 \\
& fast(rb)+pgd & 26.28 & 20.34 & 5.94 & 53.75 & 52.83 & 0.92 & 29.07 & 35.01 & -5.93 \\
& pgd(rb)+pgd  & 27.09 & 21.31 & 5.78 & 55.12 & 54.36 & 0.76 & 29.94 & 35.59 & 5.65  \\
    \midrule
    

    \multirow{3}[1]{*}{0.1}   
& sgd+pgd  & 25.38 & 22.41 & 2.97 & 53.82 & 52.87 & 0.95 & 13.31 & 15.95 & -2.65 \\
& fast+pgd & 27.24 & 23.15 & 4.09 & 55.8  & 54.79 & 1.01 & 17.2  & 21.29 & -4.09 \\
& pgd+pgd  & 26.25 & 18.62 & 7.63 & 53.18 & 51.42 & 1.76 & 31.55 & 38.55 & -6.99 \\

    \multirow{3}[1]{*}{0.1}   
& sgd(rb)+pgd  & 25.83 & 23.4  & 2.43 & 54.51 & 53.51 & 1    & 13.49 & 15.74 & -2.25 \\
& fast(rb)+pgd & 25.15 & 22.88 & 2.27 & 52.1  & 51.75 & 0.35 & 14.89 & 17.17 & -2.27 \\
& pgd(rb)+pgd  & 25.45 & 22.96 & 2.49 & 53.51 & 53.27 & 0.24 & 14.59 & 17    & -2.41 \\
    \midrule
    


    \multirow{3}[1]{*}{0.05}   
& sgd+pgd  & 25.04 & 23.29 & 1.75 & 51.5  & 50.89 & 0.61 & 5.94  & 7.61  & -1.66 \\
& fast+pgd & 26.05 & 24.49 & 1.56 & 54.09 & 53.45 & 0.64 & 7.52  & 9.09  & -1.56 \\
& pgd+pgd  & 25.21 & 22.49 & 2.72 & 51.86 & 51.39 & 0.47 & 12.14 & 14.75 & -2.61 \\

    \multirow{3}[1]{*}{0.05} 
& sgd(rb)+pgd  & 25.04 & 24.12 & 0.92 & 51.05 & 50.89 & 0.16 & 6.37  & 6.88  & -0.51 \\
& fast(rb)+pgd & 23.71 & 22.46 & 1.25 & 43.19 & 43.19 & 0    & 5.64  & 6.87  & -1.23 \\
& pgd(rb)+pgd  & 24.9  & 23.77 & 1.13 & 51.12 & 50.65 & 0.47 & 6.88  & 7.52  & -0.64 \\


    \midrule

    \bottomrule
    \end{tabular}}
  \label{tab:rb_ticket_c100}%
\end{table}%

==> Tables/table/wrn.tex <==
\begin{table}[htb]
  \centering
  \caption{Appendix: CIFAR-10, Wide-ResNet}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|l|ccc|ccc|ccc|cc}
    \toprule
    \multirow{2}[2]{*}{Sparsity(\%)} & \multirow{2}[2]{*}{Settings} & \multicolumn{3}{c|}{Generalization Gap} & \multicolumn{3}{c|}{Robust Accuracy} & \multicolumn{3}{c|}{Standard Accuracy} & \multicolumn{2}{c}{FLOPs  $\times 10^{17}$} \\
    & &  Best & Final & Diff. & Best & Final & Diff. & Best & Final & Diff.& Training & Inference \\\midrule
    $0$ & Baseline & & & & $54.73$ & $46.83$ & $7.90$ & $84.08$ & $85.84$ & $-1.76$ \\\midrule
    \multirow{2}[2]{*}{$80$} 
        & Robust Bird & & & & & & & & & \\
        & Flying Bird & & & & $55.34$ & $46.79$ & $8.55$ & $83.76$ & $85.93$ & $-2.17$ \\
    $80 \to 91.81$  & Flying Bird+ & & & & $55.34$ & $46.82$ & $8.52$ & $83.76$ & $85.97$ & $-2.21$ \\\midrule
    \multirow{2}[2]{*}{$90$} 
        & Robust Bird & & & & & & & & & \\
        & Flying Bird & & & & $54.27$ & $46.16$ & $8.11$ & $85.44$ & $86.01$ & $-0.57$ \\
    $90 \to 96.14$  & Flying Bird+ & & & & $54.24$ & $46.91$ & $7.33$ & $85.52$ & $85.93$ & $-0.41$ \\
    \bottomrule
    \end{tabular}}
  \label{tab:appendix_c10_wideres}%
\end{table}%

==> Tables/vgg16_cifar10.tex <==
% Table generated by Excel2LaTeX from sheet 'vgg16_cifar10'
\begin{table}[htbp]
  \centering
  \caption{VGG16 Cifar10}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|ccc|ccc|ccc|c}
    \toprule
    \multirow{2}[2]{*}{Density} & \multirow{2}[2]{*}{Setting} & \multicolumn{3}{c|}{Roubst Accuarcy(RA)} & \multicolumn{3}{c|}{Standard Accuarcy(RA)} & \multicolumn{3}{c|}{Generalization Gap} & \multirow{2}[2]{*}{final density(\%)} \\
          &       & Best  & Final & Diff. & Best  & Final & Diff. & Best  & Final & Diff. &  \\
    \midrule
    1     & dense & 48.33 & 42.73 & 5.6   & 76.84 & 79.73 & -2.89 & 5.72  & 27.86 & -22.14 & 100 \\
    \midrule
    \multirow{8}[1]{*}{0.2} & omp   & 47.9  & 43.19 & 4.71  & 76.6  & 80.02 & -3.42 & 4.69  & 24.97 & -20.28 & 20 \\
          & rp    & 46.14 & 40.33 & 5.81  & 74.42 & 76.68 & -2.26 & 3.94  & 21.33 & -17.39 & 20 \\
          & snip  & 48.03 & 43.17 & 4.86  & 76.68 & 80.08 & -3.4  & 4.87  & 23.49 & -18.62 & 20 \\
          & grasp & 47.91 & 42.34 & 5.57  & 75.74 & 78.87 & -3.13 & 4.16  & 21.45 & -17.29 & 20 \\
          & synflow & 48.47 & 45.32 & 3.15  & 77.62 & 79.09 & -1.47 & 5.17  & 19.46 & -14.29 & 20 \\
          & igq   & 48.57 & 44.25 & 4.32  & 77.51 & 80.01 & -2.5  & 4.84  & 21.05 & -16.21 & 20 \\
          &  dst gradient & 48.43 & 44.65 & 3.78  & 77.53 & 79.72 & -2.19 & 5.38  & 20.78 & -15.4 & 19.99 \\
          & flying & 48.25 & 45.24 & 3.01  & 77.48 & 79.55 & -2.07 & 5.57  & 18.02 & -12.45 & 10.9 \\
    \midrule
    \multirow{8}[2]{*}{0.1} & omp   & 47.84 & 43.34 & 4.5   & 75.6  & 79.1  & -3.5  & 3.42  & 18.78 & -15.36 & 10 \\
          & rp    & 44.33 & 40.33 & 4     & 71.27 & 74.46 & -3.19 & 3.06  & 14.4  & -11.34 & 10 \\
          & snip  & 47.76 & 44.27 & 3.49  & 75.92 & 79.62 & -3.7  & 3.92  & 16.93 & -13.01 & 10 \\
          & grasp & 45.96 & 42.12 & 3.84  & 75.19 & 77.03 & -1.84 & 5.03  & 16.25 & -11.22 & 10 \\
          & synflow & 47.54 & 45.79 & 1.75  & 78.43 & 78.7  & -0.27 & 9.66  & 12.71 & -3.05 & 10 \\
          & igq   & 47.79 & 45.12 & 2.67  & 74.87 & 79.19 & -4.32 & 2.72  & 14.58 & -11.86 & 10 \\
          &  dst gradient & 48.45 & 45.55 & 2.9   & 75.82 & 79.21 & -3.39 & 3.91  & 16.58 & -12.67 & 9.99 \\
          & flying & 48.39 & 46.26 & 2.13  & 78.73 & 79.12 & -0.39 & 9.29  & 12.42 & -3.13 & 4.56 \\
    \bottomrule
    \end{tabular}}
  \label{tab:addlabel}%
\end{table}%


==> Tables/vgg16_cifar100.tex <==
% Table generated by Excel2LaTeX from sheet 'vgg16_cifar100'
\begin{table}[htbp]
  \centering
  \caption{VGG16 Cifar100}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|ccc|ccc|ccc|c}
    \toprule
    \multirow{2}[2]{*}{Density} & \multirow{2}[2]{*}{Setting} & \multicolumn{3}{c|}{Roubst Accuarcy(RA)} & \multicolumn{3}{c|}{Standard Accuarcy(RA)} & \multicolumn{3}{c|}{Generalization Gap} & \multirow{2}[2]{*}{final density(\%)} \\
          &       & Best  & Final & Diff. & Best  & Final & Diff. & Best  & Final & Diff. &  \\
    \midrule
    1     & dense & 22.76 & 18.06 & 4.7   & 46.11 & 46.88 & -0.77 & 7.2   & 60.88 & -53.68 & 100 \\
    \midrule
    \multirow{8}[1]{*}{0.2} & omp   & 22.98 & 16.32 & 6.66  & 45.45 & 45.96 & -0.51 & 5.54  & 54.27 & -48.73 & 20 \\
          & rp    & 22.38 & 15.76 & 6.62  & 41.79 & 44.85 & -3.06 & 1.99  & 51.7  & -49.71 & 20 \\
          & snip  & 23.34 & 17.83 & 5.51  & 46.58 & 48.55 & -1.97 & 6.05  & 40.51 & -34.46 & 20 \\
          & grasp & 23.05 & 16.5  & 6.55  & 43.01 & 46.84 & -3.83 & 1.71  & 49.31 & -47.6 & 20 \\
          & synflow & 23.02 & 17.67 & 5.35  & 45.55 & 47.33 & -1.78 & 5.9   & 42.02 & -36.12 & 20 \\
          & igq   & 23.6  & 17.44 & 6.16  & 45.77 & 47.43 & -1.66 & 4.79  & 46.91 & -42.12 & 20 \\
          &  dst gradient & 22.75 & 17.96 & 4.79  & 46.61 & 47.36 & -0.75 & 8.86  & 47.1  & -38.24 & 19.92 \\
          & flying & 22.92 & 19.02 & 3.9   & 47.01 & 48.11 & -1.1  & 8.61  & 34.03 & -25.42 & 8.09 \\
    \midrule
    \multirow{8}[2]{*}{0.1} & omp   & 22.18 & 17.38 & 4.8   & 44.81 & 45.63 & -0.82 & 5.64  & 38.06 & -32.42 & 10 \\
          & rp    & 21.48 & 16.33 & 5.15  & 43.1  & 44.93 & -1.83 & 5.41  & 30.98 & -25.57 & 10 \\
          & snip  & 22.92 & 20.3  & 2.62  & 48.5  & 49.05 & -0.55 & 12    & 19.96 & -7.96 & 10 \\
          & grasp & 22.17 & 17.6  & 4.57  & 44.54 & 47    & -2.46 & 5.09  & 29.61 & -24.52 & 10 \\
          & synflow & 22.58 & 18.88 & 3.7   & 43.62 & 46.73 & -3.11 & 2.94  & 24.57 & -21.63 & 10 \\
          & igq   & 22.55 & 18.56 & 3.99  & 44.96 & 48.08 & -3.12 & 4.61  & 27.44 & -22.83 & 10 \\
          &  dst gradient & 23.59 & 18.86 & 4.73  & 46.64 & 48.45 & -1.81 & 5.34  & 34.22 & -28.88 & 10 \\
          & flying & 23.31 & 20.34 & 2.97  & 45.51 & 48.13 & -2.62 & 5.33  & 22.89 & -17.56 & 4.23 \\
    \bottomrule
    \end{tabular}}
  \label{tab:addlabel}%
\end{table}%


==> Tables/wide_cifar10.tex <==
% Table generated by Excel2LaTeX from sheet 'wide_cifar10'
\begin{table}[htbp]
  \centering
  \caption{WideResnet Cifar10}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|ccc|ccc|ccc|c}
    \toprule
    \multirow{2}[2]{*}{Density} & \multirow{2}[2]{*}{Setting} & \multicolumn{3}{c|}{Roubst Accuarcy(RA)} & \multicolumn{3}{c|}{Standard Accuarcy(RA)} & \multicolumn{3}{c|}{Generalization Gap} & \multirow{2}[2]{*}{final density(\%)} \\
          &       & Best  & Final & Diff. & Best  & Final & Diff. & Best  & Final & Diff. &  \\
    \midrule
    1     & dense & 54.73 & 46.83 & 7.9   & 84.08 & 85.84 & -1.76 & 10.63 & 52.17 & -41.54 & 100 \\
    \midrule
    \multirow{2}[2]{*}{0.2} &  dst gradient & 55.34 & 46.79 & 8.55  & 83.76 & 85.93 & -2.17 & 8.53  & 49.06 & -40.53 & 20 \\
          & flying & 55.34 & 46.82 & 8.52  & 83.76 & 85.97 & -2.21 & 8.53  & 46.16 & -37.63 & 8.19 \\
    \midrule
    \multirow{2}[2]{*}{0.1} &  dst gradient & 54.27 & 46.16 & 8.11  & 85.44 & 86.01 & -0.57 & 12.07 & 44.35 & -32.28 & 10 \\
          & flying & 54.24 & 46.91 & 7.33  & 85.52 & 85.93 & -0.41 & 12.1  & 38.37 & -26.27 & 3.86 \\
    \bottomrule
    \end{tabular}}
  \label{tab:addlabel}%
\end{table}%


==> ablation_batch.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[htbp]
  \centering
  \caption{The ablation study of batch size.}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|ccc|ccc|ccc|c|c}
    \toprule
    \multirow{2}[2]{*}{Batch Size} & \multicolumn{3}{c|}{Roubst Accuarcy(RA)} & \multicolumn{3}{c|}{Standard Accuarcy(RA)} & \multicolumn{3}{c|}{Generalization Gap} & \multirow{2}[2]{*}{Sparsity} & \multirow{2}[2]{*}{Total Fired Weights} \\
          & Best  & Final & Diff. & Best  & Final & Diff. & Best  & Final & Diff. &       &  \\
    \midrule
    32    & 49.81 & 48.87 & 0.94  & 80.48 & 81.03 & -0.55 & 6.25  & 8.57  & -2.32 & 7.58  & 0.54 \\
    64    & 49.15 & 47.64 & 1.51  & 82.4  & 82.45 & -0.05 & 13.44 & 15.11 & -1.67 & 9.33  & 0.59 \\
    128   & 50.99 & 48.34 & 2.65  & 79.55 & 82.69 & -3.14 & 5     & 17.82 & -12.82 & 9.45  & 0.54 \\
    256   & 50.53 & 46.96 & 3.57  & 80.91 & 82.4  & -1.49 & 8.57  & 21.64 & -13.07 & 10.85 & 0.44 \\
    512   & 49.27 & 46.16 & 3.11  & 80.2  & 81.9  & -1.7  & 10.95 & 20.95 & -10   & 10.14 & 0.32 \\
    \bottomrule
    \end{tabular}}
  \label{tab:addlabel}%
\end{table}%


==> ablation_fre.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[htbp]
  \centering
  \caption{The ablation study of sparsity update frequency.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|ccc|ccc|ccc|c|c}
    \toprule
    \multirow{2}[2]{*}{ Frequency} & \multicolumn{3}{c|}{Roubst Accuarcy(RA)} & \multicolumn{3}{c|}{Standard Accuarcy(RA)} & \multicolumn{3}{c|}{Generalization Gap} & \multirow{2}[2]{*}{Sparsity} & \multirow{2}[2]{*}{Total Fired Weights} \\
          & Best  & Final & Diff. & Best  & Final & Diff. & Best  & Final & Diff. &       &  \\
    \midrule
    100   & 50.32 & 49.02 & 1.3   & 81.28 & 81.99 & -0.71 & 10.23 & 12.16 & -1.93 & 3.94  & 0.77 \\
    500   & 50.57 & 48.37 & 2.2   & 79.76 & 82.73 & -2.97 & 5.83  & 17.45 & -11.62 & 9.17  & 0.63 \\
    1000 & 50.99 & 48.34 & 2.65  & 79.55 & 82.69 & -3.14 & 5     & 17.82 & -12.82 & 9.45  & 0.54 \\
    2000  & 51.19 & 48.39 & 2.8   & 79.8  & 83    & -3.2  & 4.5   & 17.79 & -13.29 & 9.68  & 0.43 \\
    5000  & 50.39 & 48.49 & 1.9   & 79.11 & 82.58 & -3.47 & 4.55  & 16.54 & -11.99 & 9.59  & 0.29 \\
    10000 & 50.08 & 48.02 & 2.06  & 79.25 & 82.5  & -3.25 & 5.1   & 16.08 & -10.98 & 10.01 & 0.21 \\
    \bottomrule
    \end{tabular}}
  \label{tab:addlabel}%
\end{table}%


==> ablation_init.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[htbp]
  \centering
  \caption{The ablation study of sparsity initialization.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|ccc|ccc|ccc|c|c}
    \toprule
    \multirow{2}[2]{*}{Initialization} & \multicolumn{3}{c|}{Roubst Accuarcy(RA)} & \multicolumn{3}{c|}{Standard Accuarcy(RA)} & \multicolumn{3}{c|}{Generalization Gap} & \multirow{2}[2]{*}{Sparsity} & \multirow{2}[2]{*}{Total Fired Weights} \\
          & Best  & Final & Diff. & Best  & Final & Diff. & Best  & Final & Diff. &       &  \\
    \midrule
    Uniform & 49.33 & 45.97 & 3.36  & 78.84 & 81.09 & -2.25 & 5.63  & 19.9  & -14.27 & 9.67  & 0.67 \\
    Snip  & 51    & 48.52 & 2.48  & 79.81 & 82.84 & -3.03 & 4.6   & 17.86 & -13.26 & 10.15 & 0.41 \\
    Igq   & 50.99 & 48.34 & 2.65  & 79.55 & 82.69 & -3.14 & 5     & 17.82 & -12.82 & 9.45  & 0.54 \\
    fixed ERK & 50.16 & 47.78 & 2.38  & 79.37 & 82.25 & -2.88 & 5.77  & 18.44 & -12.67 & 9.59  & 0.59 \\
    SynFlow & 50.34 & 46.86 & 3.48  & 78.67 & 81.86 & -3.19 & 4.22  & 17.44 & -13.22 & 9.59  & 0.49 \\
    \bottomrule
    \end{tabular}
    }
  \label{tab:addlabel}%
\end{table}%


==> init.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|c|rrr|rrr|rrr|r|r|}
\cmidrule{1-10}\cmidrule{12-12}    \multirow{2}[2]{*}{Initialization} & \multicolumn{3}{c|}{Roubst Accuarcy(RA)} & \multicolumn{3}{c|}{Standard Accuarcy(RA)} & \multicolumn{3}{c|}{Generalization Gap} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Sparsity}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Total Fired Weights}} \\
          & \multicolumn{1}{c}{Best} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c|}{Diff.} & \multicolumn{1}{c}{Best} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c|}{Diff.} & \multicolumn{1}{c}{Best} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c|}{Diff.} &       &  \\
    \midrule
    Uniform & 49.33 & 45.97 & 3.36  & 78.84 & 81.09 & -2.25 & 5.63  & 19.9  & -14.27 & 9.67  & 0.67 \\
\cmidrule{1-1}    Snip  & 51    & 48.52 & 2.48  & 79.81 & 82.84 & -3.03 & 4.6   & 17.86 & -13.26 & 10.15 & 0.41 \\
\cmidrule{1-1}    Igq   & 50.99 & 48.34 & 2.65  & 79.55 & 82.69 & -3.14 & 5     & 17.82 & -12.82 & 9.45  & 0.54 \\
\cmidrule{1-1}    fixed ERK & 50.16 & 47.78 & 2.38  & 79.37 & 82.25 & -2.88 & 5.77  & 18.44 & -12.67 & 9.59  & 0.59 \\
\cmidrule{1-1}    SynFlow & 50.34 & 46.86 & 3.48  & 78.67 & 81.86 & -3.19 & 4.22  & 17.44 & -13.22 & 9.59  & 0.49 \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> static_grasp.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[htbp]
  \centering
  \caption{Performance of experiments using Grasp as the sparsity initialization method.}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cccccc|cccccc|cccccc}
    \toprule
    \multirow{3}[2]{*}{Density} & \multicolumn{6}{c|}{Roubst Accuarcy(RA)}      & \multicolumn{6}{c|}{Standard Accuarcy(RA)}    & \multicolumn{6}{c}{Generalization Gap} \\
          & \multicolumn{2}{c}{ Best} & \multicolumn{2}{c}{ Final} & \multicolumn{2}{c|}{ Diff.} & \multicolumn{2}{c}{ Best} & \multicolumn{2}{c}{ Final} & \multicolumn{2}{c|}{ Diff.} & \multicolumn{2}{c}{ Best} & \multicolumn{2}{c}{ Final} & \multicolumn{2}{c}{ Diff.} \\
          & mean  & std   & mean  & std   & mean  & std   & mean  & std   & mean  & std   & mean  & std   & mean  & std   & mean  & std   & mean  & std \\
    \midrule
    0.05  & 48.2  & 0.34  & 46.38 & 0.68  & 1.82  & 0.4   & 78.91 & 0.04  & 79.46 & 0.03  & -0.55 & 0.06  & 6.79  & 0.25  & 9.75  & 0.78  & -2.96 & 0.94 \\
    0.1   & 48.76 & 0.21  & 45.97 & 0.77  & 2.79  & 0.9   & 78.41 & 0.53  & 81.32 & 0.09  & -2.91 & 0.47  & 4.54  & 0.66  & 16.17 & 0.71  & -11.63 & 1.36 \\
    0.2   & 49.79 & 0.38  & 44.69 & 0.59  & 5.1   & 0.49  & 78.87 & 0.67  & 82.29 & 0.58  & -3.42 & 0.54  & 5.4   & 0.89  & 24.86 & 0.61  & -19.47 & 0.72 \\
    0.6   & 50.92 & 0.3   & 42.49 & 0.69  & 8.43  & 0.56  & 80.24 & 0.3   & 82.41 & 0.36  & -2.17 & 0.11  & 6.85  & 0.63  & 38.73 & 0.84  & -31.88 & 1.2 \\
    0.8   & 51.18 & 0.5   & 42.46 & 0.47  & 8.72  & 0.61  & 80.99 & 0.62  & 83.04 & 0.25  & -2.04 & 0.6   & 7.53  & 1.63  & 40.99 & 0.52  & -33.46 & 1.73 \\
    \bottomrule
    \end{tabular}}
  \label{tab:addlabel}%
\end{table}%


==> static_snip.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Performance of experiments using SNIP as the sparsity initialization method.}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cccccc|cccccc|cccccc}
    \toprule
    \multirow{3}[2]{*}{Density} & \multicolumn{6}{c|}{Roubst Accuarcy(RA)}      & \multicolumn{6}{c|}{Standard Accuarcy(RA)}    & \multicolumn{6}{c}{Generalization Gap} \\
          & \multicolumn{2}{c}{ Best} & \multicolumn{2}{c}{ Final} & \multicolumn{2}{c|}{ Diff.} & \multicolumn{2}{c}{ Best} & \multicolumn{2}{c}{ Final} & \multicolumn{2}{c|}{ Diff.} & \multicolumn{2}{c}{ Best} & \multicolumn{2}{c}{ Final} & \multicolumn{2}{c}{ Diff.} \\
          & mean  & std   & mean  & std   & mean  & std   & mean  & std   & mean  & std   & mean  & std   & mean  & std   & mean  & std   & mean  & std \\
    \midrule
    0.05  & 47.88 & 0.39  & 46.29 & 0.74  & 1.59  & 0.38  & 78.55 & 1.09  & 79.55 & 0.39  & -1.01 & 0.88  & 6.96  & 0.9   & 9.09  & 0.77  & -2.12 & 0.31 \\
    0.1   & 49.5  & 0.08  & 47.1  & 0.65  & 2.41  & 0.67  & 79.28 & 1.89  & 82.03 & 0.25  & -2.75 & 2     & 5.8   & 4.06  & 15.44 & 0.92  & -9.64 & 3.77 \\
    0.2   & 50.22 & 0.29  & 45.7  & 0.68  & 4.52  & 0.61  & 80.45 & 0.28  & 83.47 & 0.35  & -3.02 & 0.29  & 6.69  & 0.99  & 24.39 & 0.93  & -17.7 & 0.42 \\
    0.6   & 51.72 & 0.35  & 43.14 & 0.61  & 8.59  & 0.47  & 80.86 & 0.12  & 83.44 & 0.12  & -2.58 & 0.03  & 6.58  & 0.35  & 38.9  & 0.66  & -32.32 & 0.88 \\
    0.8   & 51.68 & 0.4   & 43.22 & 0.42  & 8.45  & 0.33  & 81.98 & 0.53  & 83.55 & 0.04  & -1.58 & 0.5   & 8.37  & 1.01  & 41.03 & 0.37  & -32.67 & 0.69 \\
    \bottomrule
    \end{tabular}}
  \label{tab:addlabel}%
\end{table}%


==> static_synflow.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[htbp]
  \centering
  \caption{Performance of experiments using SynFlow as the sparsity initialization method.}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cccccc|cccccc|cccccc}
    \toprule
    \multirow{3}[2]{*}{Density} & \multicolumn{6}{c|}{Roubst Accuarcy(RA)}      & \multicolumn{6}{c|}{Standard Accuarcy(RA)}    & \multicolumn{6}{c}{Generalization Gap} \\
          & \multicolumn{2}{c}{ Best} & \multicolumn{2}{c}{ Final} & \multicolumn{2}{c|}{ Diff.} & \multicolumn{2}{c}{ Best} & \multicolumn{2}{c}{ Final} & \multicolumn{2}{c|}{ Diff.} & \multicolumn{2}{c}{ Best} & \multicolumn{2}{c}{ Final} & \multicolumn{2}{c}{ Diff.} \\ 
          & mean  & std   & mean  & std   & mean  & std   & mean  & std   & mean  & std   & mean  & std   & mean  & std   & mean  & std   & mean  & std \\
    \midrule
    0.05  & 48.74 & 0.2   & 47.62 & 0.64  & 1.13  & 0.6   & 78.26 & 0.57  & 79    & 0.46  & -0.74 & 0.47  & 5.78  & 0.59  & 7.83  & 0.76  & -2.05 & 0.61 \\
    0.1   & 49.92 & 0.37  & 47.57 & 0.42  & 2.34  & 0.3   & 81.05 & 0.13  & 81.67 & 0.47  & -0.62 & 0.41  & 10.04 & 0.85  & 13.94 & 0.5   & -3.9  & 0.94 \\
    0.2   & 50.79 & 0.39  & 46.27 & 0.57  & 4.52  & 0.23  & 79.35 & 0.35  & 83.08 & 0.19  & -3.73 & 0.53  & 4.25  & 0.37  & 23.31 & 0.71  & -19.07 & 0.63 \\
    0.6   & 51.52 & 0.2   & 43.61 & 0.42  & 7.91  & 0.27  & 81.04 & 0.14  & 83.32 & 0.33  & -2.28 & 0.36  & 7.26  & 1.19  & 37.95 & 0.35  & -30.69 & 1.22 \\
    0.8   & 51.58 & 0.19  & 43.65 & 0.79  & 7.93  & 0.75  & 81.08 & 0.14  & 83.36 & 0.33  & -2.28 & 0.4   & 7.09  & 0.58  & 39.69 & 0.78  & -32.6 & 1.35 \\
    \bottomrule
    \end{tabular}}
  \label{tab:addlabel}%
\end{table}%

